Contextuality in distributed systems

We present a lattice of distributed program specifications, whose ordering represents implementability/refinement. Specifications are modelled by families of subsets of relative execution traces, which encode the local orderings of state transitions, rather than their absolute timing according to a global clock. This is to overcome fundamental physical difficulties with synchronisation. The lattice of specifications is assembled and analysed with several established mathematical tools. Sets of nondegenerate cells of a simplicial set are used to model relative traces, presheaves model the parametrisation of these traces by a topological space of variables, and information algebras reveal novel constraints on program correctness. The latter aspect brings the enterprise of program specification under the widening umbrella of contextual semantics introduced by Abramsky et al. In this model of program specifications, contextuality manifests as a failure of a consistency criterion comparable to Lamport's definition of sequential consistency. The theory of information algebras also suggests efficient local computation algorithms for the verification of this criterion. The novel constructions in this paper have been verified in the proof assistant Isabelle/HOL.

==> content/excluded.tex <==
\section{Stuff that is not in the paper but will go in the thesis}

\subsection{Monoidal preorder structure}

\todo{probably exclude this subsection}

\subsection{Local concurrent Kleene algebra structure}

\todo{remove this subsection if not enough space and mention the construction in the discussion}

We will now see that we can enrich the information algebra $(\phialg,\cat{D})$ with another operation $\seq : \phialg \times \phialg \to \phialg$ that represents the \emph{sequential composition} of computations.

Let $U \in \cat{D}$ be fixed.

We define \defn{concatenation} of traces as a \emph{partially defined} operation
\[
    \concat_U : T_U \times T_U \to T_U
\]
where $f \concat_U g$ concatenates $f$ to $g$, \emph{defined when the final state of $f$ matches the initial trace of $g$}, and then removes the final state of $f$ from the concatenation.
It is easy to show that $f \concat_U g$ is then nondegenerate, and hence the operation is well-defined, and also that the operation $\concat_U$ is associative.

\todo{Show this anyway}

We lift this operation to an operation $\seq_U : \phialg_U \times \phialg_U \to \phialg_U$, by defining
\[
    R \seq_U S \defeq
    \setc{
        f \concat_U g \in T_U
    }
    {
        f \in R, g \in S, f \neq (), g \neq (), \term{f} = \init{g}
    }
\]
where $\term{f}$ denotes the final state of $f$ and $\init{g}$ the initial state of $g$.
This operation is associative, and has a unit given by the relation $S_U \in \phialg_U$ (\enquote{skip}) consisting of all length-1 traces (i.e. 0-simplices, beware of the off-by-one), and a null element given by $Z_U$.

\todo{Show this anyway}

\begin{definition}[Semiring]
    % rephrase
    A \defn{semiring} is a structure $(S,+,0,\cdot,1)$ such that $(S,+,0)$ is a commutative monoid, $(S,\cdot,1)$ is a monoid, multiplication distributes over addition in both arguments, and $0$ is a left and right annihilator with respect to multiplication, i.e. $a \cdot 0 = 0 = 0 \cdot a$.
    A semiring is \defn{idempotent} if its addition is.
\end{definition}

\begin{definition}[Quantale]
    % rephrase
    A \defn{quantale} (or \defn{Kleene algebra}) is an idempotent semiring that is a complete lattice under the natural order and in which composition distributes over arbitrary supreme, i.e.
    \begin{equation}
        \label{ch1.eqn.quantale1}
        x * \tuple{ \bigvee_{i\in I} y_i}
        = \bigvee_{i\in I} ( x * y_i)
    \end{equation}
    and
    \begin{equation}
        \label{ch1.eqn.quantale2}
        \tuple{ \bigvee_{i\in I} y_i} * x
        = \bigvee_{i\in I} ( y_i * x)
    \end{equation}

\end{definition}

\begin{definition}[Concurrent Kleene algebra]
    % rephrase
    A \defn{concurrent Kleene algebra} (CKA) is a structure $(S,+,0,*,\seq,1)$ such that $(S,+,0,*,1)$ and $(S,+,0,\seq,1)$ are quantales such that for all $a,b,c,d \in S$, the \defn{exchange law} holds,
    \begin{equation}
        \label{ch1.eqn.interchange}
        (a * b) \seq (c * d) \leq
        (a \seq c) * (b \seq d)
    \end{equation}
    \todo{in Hoare et al. the RHS is $(b \seq c) * (a \seq d)$}
\end{definition}

\begin{remark}
    The exchange law of a CKA implies monotonicity of the multiplications $*$ and $\seq$.
    \todo{does this follow just from the quantale structure?}
\end{remark}

\begin{proposition}
    For each $U \in \cat{D}$, $\phialg_U$ with the operations $* \defeq \otimes$ and $\seq \defeq \seq$ is a concurrent Kleene algebra.
\end{proposition}
\begin{proof}
    First note that $\otimes$ restricted to $\phialg_U \times \phialg_U$ is just subset intersection $\cap$.
    Then $(\phialg_U, \cap)$ is a quantale because intersections distribute over unions.

    Let $h \in
        R \seq \tuple{ \bigcup_{i\in I} S_i}
    $.
    Then
    \begin{align*}
        h & \in
        \setc{
            f \concat_U g \in T_U
        }
        {
            f \in R, g \in \bigcup_{i\in I} S_i, f \neq (), g \neq (), \term{f} = \init{g}
        }                                 \\
          & =
        \bigcup_{i\in I}
        \setc{
            f \concat_U g \in T_U
        }
        {
            f \in R, g \in S_i, f \neq (), g \neq (), \term{f} = \init{g}
        }                                 \\
          & =\bigcup_{i\in I} ( R * S_i),
    \end{align*}
    which shows~\cref{ch1.eqn.quantale1}, and~\cref{ch1.eqn.quantale2} is similar.
    Thus, $(\phialg_U, \seq)$ is a quantale.

    Let $f \in (A \cap B) \seq (C \cap D)$.
    Then $f$ can be represented by a pair $(g,h)$ where $g \in A \cap B$, $h \in C \cap D$, and $\term{g} = \init{h}$.
    Then clearly $(g,h)$ corresponds to a trace in $A \seq C$ as well as a trace in $B \seq D$, hence $f$ is in the right-hand side of~\cref{ch1.eqn.interchange}.
    This proves $\phialg_U$ is a CKA.
\end{proof}

\begin{remark}
    The inequality~\cref{ch1.eqn.interchange} is generally sharp: let $\abs{U} = 1$ and let $A = D = \set{ \trace{0}}$ and $B = C = \set {\trace{0,0}}$.
    Then $A \seq C = B \seq D = \set{[0,0]}$, so the right-hand side of~\cref{ch1.eqn.interchange} is inhabited, whereas the left-hand side is clearly empty.
\end{remark}

We can lift the definition of $\seq_U$ to an operation $\seq : \phialg \times \phialg \to \phialg$ with the following definition:
\begin{align*}
    R \seq S \defeq
    \setc{
        f \in \phialg_{d(R) \cup d(S),}
    }{
        \proj{f}{d(R) \cap d(S)}
        \in \proj{R}{U} \seq_U \proj{S}{U}
    }
\end{align*}

\todo{is there a good reason to do this?}

\todo{describe the link between the implementation preordering and the Kleene algebra structure.}

\subsection{\v{C}ech cohomology}
\todo{reduce this section to a sentence or two}
The task of detecting these problematic matching families that do not come from a global section can be tackled with linear algebra via a construction known as \defn{\v{C}ech cohomology}.
Fix a principal ideal domain $R$ (for example, the integers $\Zz$, or the field of real numbers $\Rr$, or a finite field $\Zz/p\Zz$ for a prime number $p$).

For a specification $A$ in a distributed context $\cat{U} = \set{U_i}_{i \in I}$, we construct a \loud{simplicial complex} (the higher-dimensional analog of an undirected graph) whose vertices are the $U_i$ and whose $n$-cells are nonempty $n$-fold intersections of the $U_i$, called the \loud{\v{C}ech nerve of the cover $\cat{U}$}.
This simplicial complex is a combinatorial model of the distributed context.

Now to each cell $U$ of the \v{C}ech nerve we assign the free $R$-module whose basis is $A U$, which we write as $\hat{A} U$ (when $R$ is a ring, this is a vector space.)

We can connect these $R$-modules in a sequence extending infinitely to the right
\[
    0
    \to \hat{A}(X)
    \xrightarrow{d^{-1}} \bigoplus_{i} \hat{A}(U_i)
    \xrightarrow{d^{0}}\bigoplus_{i<j}\hat{A}(U_i\cap U_j)
    \xrightarrow{d^{1}} \ldots
\]
where the arrows denote certain $R$-linear maps that satisfy
\begin{equation}
    \label{coboundary}
    \fa{p}{d^{p+1} \circ d^p = 0}
\end{equation}
This sequence of spaces and maps is called the \defn{augmented \v{C}ech complex of the cover $\cat{U}$} \cite{279243}.

Because of the property~\cref{coboundary}, the image of each map $d^p$ is contained within the kernel of $d^{p+1}$, and so we can define the quotients
\[
    H^p(\hat{A}, \cat{U}) \defeq \vker{d^{p}}/\vim{d^{p-1}}
\]
called the \defn{cohomology rings of $\hat{A}$ on $\cat{U}$ over $R$ in degree $p$}.

The first two of these rings reveal information about obstructions to correctness of the refinement of a global specification $A V$ to the distributed context $\cat{U}$: the ring $H^{-1}$ contains ($R$-linear combinations) of global sections that restrict to $0$ on the context---these are executions that fail to be parallelised; whereas the ring $H^0$ contains ($R$-linear combinations) of local sections that fail to lift to a global execution.


==> content/results.tex <==
\section{Results}
\label{sec}
% i found

